Spatial-Temporal Super-Resolution of Satellite Imagery via Conditional Pixel Synthesis

High-resolution satellite imagery has proven useful for a broad range of tasks, including measurement of global human population, local economic livelihoods, and biodiversity, among many others. Unfortunately, high-resolution imagery is both infrequently collected and expensive to purchase, making it hard to efficiently and effectively scale these downstream tasks over both time and space. We propose a new conditional pixel synthesis model that uses abundant, low-cost, low-resolution imagery to generate accurate high-resolution imagery at locations and times in which it is unavailable. We show that our model attains photo-realistic sample quality and outperforms competing baselines on a key downstream task -- object counting -- particularly in geographic locations where conditions on the ground are changing rapidly.

==> checklist.tex <==
\newpage
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section~\ref{intro}.}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{experiment},~\ref{impact}, Appendix G.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section~\ref{impact}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Section~\ref{experiment} and Appendix B.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section 5 and Appendix B.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See Section~\ref{experiment}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix B.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Section~\ref{experiment}.}
  \item Did you mention the license of the assets?
    \answerYes{See Appendix C.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See Section~\ref{experiment}, Appendix C.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See Appendix C.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{See Appendix D.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{See Appendix D.}
\end{enumerate}

\end{enumerate}

==> impact.tex <==
\section{Statement of Broader Impact}
\label{impact}

With our proposed Spatial-Temporal Super-Resolution approach, we aim to move the needle towards a more equitable social and economic environment in two ways. First, we hope that the ability to extend the availability of high resolution satellite imagery in areas where such images are temporally sparse will help narrow the data gap between regions of varying economic development and aid in decision making. On this point, we acknowledge that certain areas of the globe may still have no high resolution satellite coverage \cite{reid_2020}, in which case our approach may exacerbate the data gap by only helping regions that already have some high resolution satellite imagery. Second, we hypothesize that the presence of a high resolution temporally divergent conditional input along with the low resolution input at the desired time may help mitigate the impact of training set distribution bias. However, additional experiments are needed to evaluate this hypothesis, and our model is still expected to suffer from bias if trained on data that is not representative of the target distribution. Additionally, we acknowledge that increasing the temporal availability of high resolution satellite imagery has potential applications in surveillance. Finally, while we hope our approach can aid in large-scale downstream applications such as post-disaster building damage estimation and poverty prediction, we caution against using generated images to inform individual policy decisions (e.g. retroactively applying permit fees for swimming pools).
